A Polyhedral Study of Lifted Multicuts

Fundamental to many applications in data analysis are the decompositions of a graph, i.e. partitions of the node set into component-inducing subsets. One way of encoding decompositions is by multicuts, the subsets of those edges that straddle distinct components. Recently, a lifting of multicuts from a graph $G = (V, E)$ to an augmented graph $\hat G = (V, E \cup F)$ has been proposed in the field of image analysis, with the goal of obtaining a more expressive characterization of graph decompositions in which it is made explicit also for pairs $F \subseteq \tbinom{V}{2} \setminus E$ of non-neighboring nodes whether these are in the same or distinct components. In this work, we study in detail the polytope in $\mathbb{R}^{E \cup F}$ whose vertices are precisely the characteristic vectors of multicuts of $\hat G$ lifted from $G$, connecting it, in particular, to the rich body of prior work on the clique partitioning and multilinear polytope.

==> figures/introductory-example/base-decomposition.tex <==
\def \r {0.2cm}

\node[style=vertex] (0) at (0.0, 1.1) {};
\node[style=vertex] (1) at (0.6, 0.7) {};
\node[style=vertex] (2) at (1.7, 1.0) {};
\node[style=vertex] (3) at (0.2, -0.1) {};
\node[style=vertex] (4) at (0.9, 0.1) {};
\node[style=vertex] (5) at (1.8, -0.2) {};
\node[style=vertex] (6) at (2.5, 0.8) {};
\node[style=vertex] (7) at (2.6, 0.2) {};

\draw (0) -- (1);
\draw[style=cut-edge] (0) -- (2);
\draw[style=cut-edge] (0) -- (3);
\draw[style=cut-edge] (1) -- (3);
\draw[style=cut-edge] (1) -- (2);
\draw[style=cut-edge] (1) -- (4);
\draw[style=cut-edge] (1) -- (5);
\draw (2) -- (4);
\draw[style=cut-edge] (2) -- (5);
\draw (3) -- (4);
\draw[style=cut-edge] (3) -- (5);
\draw[style=cut-edge] (4) -- (5);
\draw (5) -- (7);
\draw (6) -- (7);
\draw (5) -- (6);
\draw[style=cut-edge] (6) -- (2);

\path[fill=mygreen,draw=mygreen,opacity=0.3,line width=4ex,line cap=round,line join=round]
    (3)--(4)--(2)--cycle;

\path[fill=mygreen,draw=mygreen,opacity=0.3,line width=4ex,line cap=round,line join=round]
    (5)--(7)--(6)--(5);

\path[fill=mygreen,draw=mygreen,opacity=0.3,line width=4ex,line cap=round,line join=round]
    (0)--(1);

% label selected nodes
\node[draw=none] at (0, 1.4) {$u$};
\node[draw=none] at (1.45, 1.2) {$v$};
\node[draw=none] at (2.5, 1.1) {$w$};

% draw invisible lifted edge to ensure that both figures have same bounding box
\draw[opacity=0] (0) edge[bend left=40] (6);
